GenBFA: An Evolutionary Optimization Approach to Bit-Flip Attacks on LLMs

Large Language Models (LLMs) have revolutionized natural language processing (NLP), excelling in tasks like text generation and summarization. However, their increasing adoption in mission-critical applications raises concerns about hardware-based threats, particularly bit-flip attacks (BFAs). BFAs, enabled by fault injection methods such as Rowhammer, target model parameters in memory, compromising both integrity and performance. Identifying critical parameters for BFAs in the vast parameter space of LLMs poses significant challenges. While prior research suggests transformer-based architectures are inherently more robust to BFAs compared to traditional deep neural networks, we challenge this assumption. For the first time, we demonstrate that as few as three bit-flips can cause catastrophic performance degradation in an LLM with billions of parameters. Current BFA techniques are inadequate for exploiting this vulnerability due to the difficulty of efficiently identifying critical parameters within the immense parameter space. To address this, we propose AttentionBreaker, a novel framework tailored for LLMs that enables efficient traversal of the parameter space to identify critical parameters. Additionally, we introduce GenBFA, an evolutionary optimization strategy designed to refine the search further, isolating the most critical bits for an efficient and effective attack. Empirical results reveal the profound vulnerability of LLMs to AttentionBreaker. For example, merely three bit-flips (4.129 x 10^-9% of total parameters) in the LLaMA3-8B-Instruct 8-bit quantized (W8) model result in a complete performance collapse: accuracy on MMLU tasks drops from 67.3% to 0%, and Wikitext perplexity skyrockets from 12.6 to 4.72 x 10^5. These findings underscore the effectiveness of AttentionBreaker in uncovering and exploiting critical vulnerabilities within LLM architectures.

==> sections/backup.tex <==
\section{Proposed Methodology}\label{sec:methodology}
In this section, we commence by delineating the threat model, which articulates the standard assumptions concerning the adversary’s capabilities. Subsequently, we introduce an innovative BFA framework specifically targeting LLMs. This framework identifies and manipulates the most critical weights within the pre-trained models, precipitating a substantial degradation in model performance.
\subsection{Threat Model}
In the realm of Machine Learning as a Service (MLaaS), the deployment of LLMs on shared computational platforms introduces significant security vulnerabilities. These platforms, while providing enhanced computational resources, expose LLMs to potential BFAs due to shared hardware components such as last-level caches and main memory. Attackers, even without explicit permissions to access user data, can exploit side channels to induce bit-flips in the memory cells storing the LLM's parameters. This threat model categorizes the risks into three levels based on the attacker's knowledge and access. (1) At the basic level, attackers can cause minor perturbations, degrading model performance. (2) Intermediate attackers can target specific bits, significantly impairing model accuracy. (3) Advanced attackers, with sophisticated techniques, can induce catastrophic failures, including complete model corruption or the introduction of backdoors. %The extreme severity of these attacks necessitates robust security measures at both hardware and software levels to ensure the integrity and reliability of LLMs in MLaaS environments. Effective mitigation strategies may include hardware-level protections, continuous monitoring, and anomaly detection systems to safeguard against these pervasive threats.
%\subsection{Attack Setup}
%In this section, we present the setup for a BFA on a LLM stored in memory, a vulnerability that poses significant threats to the model's integrity and reliability. 

In this scenario, an attacker with elevated privileges gains unauthorized access to the memory where the LLM's weights are stored. By exploiting a BFA method, such as the RowHammer attack~\cite{mutlu2019rowhammer}, the attacker selectively flips critical bits in the model's weights. This alteration is often imperceptible to the user, with the model's outputs appearing to be superficially correct. However, the underlying model has been compromised, potentially leading to erratic and erroneous results. Such an attack undermines the model's reliability, especially in mission-critical applications, including healthcare, finance, and autonomous systems.

%Studies have demonstrated that BFAs can severely degrade the performance of neural networks by corrupting the parameters stored in memory. These attacks exploit memory cell vulnerabilities to induce faults, resulting in substantial accuracy degradation or the introduction of malicious functionalities. The consequences of these attacks are profound, as they can either incapacitate the model or cause it to behave unpredictably, posing significant risks to any system reliant on the compromised model. Consequently, it is imperative to develop resilient defense mechanisms and conduct comprehensive security evaluations to safeguard LLMs against such adversarial threats.
\iffalse
\subsection{Model parameter sensitivity analysis: Magnitude vs Gradient}\label{sec:magVsgrad}
The sensitivity of model weights in neural networks, including Convolutional Neural Networks (CNNs), Recurrent Neural Networks (RNNs), and Large Language Models (LLMs), is influenced by both their absolute magnitudes and gradients, which reflect their impact on model loss. This sensitivity can vary significantly based on the precision of the model.

In full-precision models (\textit{e.g.}, float32), weights can range between approximately \(-3.4 \times 10^{38}\) and \(3.4 \times 10^{38}\). In such models, even a single bit-flip can introduce substantial errors, particularly for weights with large magnitudes. This is because the large range of representable values makes the model highly sensitive to bit-flip-induced errors. The sensitivity of weights in this context is primarily magnitude-based, as larger weights are more susceptible to errors. For a weight \( w \) with a large magnitude, the sensitivity \( S_{\text{mag}} \) can be approximated as $S_{\text{mag}} \propto |w|$. This indicates that weights with larger magnitudes are more sensitive to perturbations.

However, sensitivity derived from gradients may not always align with magnitude-based sensitivity. Gradients capture different aspects of the model's behavior, reflecting how changes in weights affect the loss function. For instance, a weight with a small magnitude but a large gradient can have a significant impact on the model's performance. Therefore, gradient-based sensitivity provides a complementary perspective to magnitude-based sensitivity. For a weight \( w \) with a gradient \( \nabla L(w) \), the sensitivity \( S_{\text{grad}} \) can be approximated as $S_{\text{grad}} \propto |\nabla L(w)|$. This indicates that weights with larger gradients are more sensitive to changes in the loss function.

As model precision decreases, from fp16 to int8, int4, or even down to 3-bit, 2-bit, and binary representations, the potential for error from bit-flips diminishes because the range of representable values narrows. Therefore, gradient-based sensitivity becomes increasingly important, as it is not strictly tied to weight magnitude and can capture more nuanced variations in model behavior.

Therefore, in practice, both magnitude and gradient-based sensitivities should be considered. The combined sensitivity \( S \) can be expressed as:
\begin{equation}\label{eq:sensitivity}
    S \propto \alpha|w| + (1-\alpha)|\nabla L(w)|
\end{equation}
, where $\alpha$ is a tunable parameter. Therefore, we employ this weighted approach to identify sensitive parameters in the model.
\fi
\subsection{Proposed Attack Framework}
Here, we propose an attack framework comprising four structured steps: (1) Layer Sensitivity Analysis, which generates a sensitivity profile for each layer; (2) Weight Subset Selection, which extracts a critical subset of weights from this profile; (3) Weight Subset Optimization, which refines this subset to identify the model’s most vulnerable weight set; and (4) iterative pruning to further narrow down to the most critical bits in the whole model for efficient BFA. 
\subsubsection{Layer sensitivity analysis}\label{sec:layer_sensitivity}
% In this section, we elucidate the necessity of ranking model layers according to their sensitivity, alongside the methodology employed for this purpose. 
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/Experiments-AttnBreaker-Venn.pdf}
    \caption{Critical parameter identification process using step-wise optimizations for efficient BFA on LLMs.}
    \label{fig:venn}
\end{figure}
Prior research has demonstrated that the sensitivity to hardware faults or computational errors varies significantly across different layers of neural network models, thereby causing non-uniform impacts on model performance~\cite{kundubit}. To systematically identify critical parameters, it is essential to reduce the parameter search space by focusing on layers with the highest sensitivity, thus motivating a ranking of layers based on susceptibility to perturbations.

Let us define an  $L$-layer model $\mathcal{M}$ parameterized by $\mathbf{W}$. For each layer \( l \), we define the top-\( k \) parameters by selecting weights \( w_i \) according to their   sensitivity score calculated using Equation \ref{eq:sensitivity}:
\begin{equation}
    \mathbf{S} = \alpha \cdot |\nabla \mathbf{W}_N| + (1 - \alpha) \cdot |\mathbf{W}_N|
    \label{eq:sensitivity}
\end{equation}

where \( \alpha \in [0,1] \) is the sensitivity ratio (a weighting parameter) to balance gradient and magnitude contributions. $\mathbf{W}_N$ refers to normalized model weights ($\mathbf{W}$) and $\nabla \mathbf{W}_N$ refers to normalized model gradients ($\nabla \mathbf{W}$).
\(\alpha = 0\) emphasizes weight magnitudes, \(\alpha = 1\) emphasizes gradients, and intermediate values adjust the balance. 

For each weight \(w_i\), this scoring function  thus quantifies sensitivity by combining both the parameter’s magnitude and gradient information. The weights are collated and sorted in descending order of of their sensitivity \(S(w_i)\), yielding a prioritized list of the most critical weights in the selected layers. 
Now in order to analyze the sensitivity of each layer, top-\( k \) weights \( w_i \) from the layer based on their sensitivy scores are selected for perturbation. Specifically, \( k \) is defined as:
\begin{equation}\label{eq:topk}
    k = \texttt{cardinality}(\mathbf{W}^{(l)}) \times \frac{r}{100}
\end{equation}
where $s$ is the sub-sampling rate refering to what percentage of parameters are selected and \texttt{cardinality} is a function providing the total number of parameters in $\mathbf{W}^{(l)}$.
For inducing highest impact this perturbation is applied by flipping the most significant bit (MSB) ($w_i' = w_i \oplus 2^{\text{MSB}}$) or the sign bit ($w_i' = -w_i$).
The resultant model loss $\mathcal{L}$ is calculated post-perturbation, and the sensitivity of layer is quantified by its corresponding perterbation loss $\mathcal{L}_l$. 



%In this section, we outline the necessity for ranking model layers based on sensitivity and the methodology employed. Prior research indicates that sensitivity to faults varies across neural network layers, leading to differential impacts on model performance. To identify critical parameters, we reduce the search space by focusing on the most sensitive layers, necessitating a systematic ranking process. We employ a top-(k) weight perturbation technique for each layer, selecting top-(k) weights based on absolute magnitudes and gradients. These weights are perturbed by flipping the most significant bit (MSB) ($w_i' = w_i \oplus 2^{\text{MSB}}$) or the sign bit ($w_i' = -w_i$), followed by the calculation of model loss. Layer sensitivity is quantified as the change in loss ($\Delta L = L' - L$), allowing us to rank layers based on the resulting \(\Delta L\), yielding gradient-based ranking \(R_{grad}\) and magnitude-based ranking \(R_{mag}\).

\begin{algorithm}[t]
\caption{Layer Sensitivity Analysis}
\begin{algorithmic}[1]
\Require An  $L$-layer model $\mathcal{M}$ parameterized by $\mathbf{W}$, gradient $\nabla \mathbf{W}$, $\alpha$, sub-sampling $\%$  $r$ 
\State \text{Initialize sensitivity loss:} $\mathcal{L}_{\text{sens}} = [\text{ }]$
\Function{\texttt{SScore}}{$|\mathbf{W}|$, $|\nabla \mathbf{W}|$, $\alpha$}
    \State $|\mathbf{W}_N| \gets \texttt{Normalize}(|\mathbf{W}|)$
    \State $|\nabla \mathbf{W}_N| \gets \texttt{Normalize}(|\nabla \mathbf{W}|)$
    \State $\mathbf{S} \gets \alpha \cdot |\nabla \mathbf{W}_N| + (1 - \alpha) \cdot |\mathbf{W}_N|$
    \State \Return $\mathbf{S}$
\EndFunction
\Function{\texttt{BFLIP}}{$\mathbf{W}^{(l)}$, $pos$, $I$}
        \State $\mathbf{W}^{(l)}_{orig} \gets \mathbf{W}^{(l)}$
        \ForAll{$i \in I$}
        \State $w^{(l)}_i \gets w^{(l)}_i \oplus (1 \ll pos)$
        % \If{$L' \geq L_{th}$} 
        %     \State W_{critical}$\gets W_k[flipped]$
        %     \State \textbf{Break}
        % \EndIf 
    \EndFor
    \State $\mathcal{M} \gets \texttt{updateModel}(\mathcal{M}, \mathbf{W}^{(l)})$
    \State $\mathcal{L} \leftarrow \texttt{ComputeLoss}(\mathcal{M})$
    \State $\mathcal{M} \gets \texttt{updateModel}(\mathcal{M}, \mathbf{W}^{(l)}_{orig})$
    \State \Return $\mathcal{L}$
\EndFunction

\ForAll{$l \in L$}
    \State $k \gets r*\texttt{cardinality}(\mathbf{W}^{(l)})/100$
    %\State $I^{(l)}_{\text{mag}} \gets \texttt{Top$k$Index}(|\mathbf{W}^{(l)}|)$
    %\State $I^{(l)}_{\text{grad}} \gets \texttt{Top$k$Index}(|\nabla \mathbf{W}^{(l)}|)$
    \State $\textbf{S}^{(l)}$$\gets$ \texttt{SScore}($|\mathbf{W}^{(l)}|$, $|\nabla \mathbf{W}^{(l)}|$, $\alpha$)
    \State $I^{(l)}_{\text{hybrid}} \gets \texttt{Top$k$Index}(\mathbf{S}^{(l)})$
    
    \State $\mathcal{L}^{(l)}_p \leftarrow \texttt{BFLIP}({\mathbf{W}^{(l)}, pos, I^{(l)}_{\text{hybrid}}})$
    \State \text{Push} $\mathcal{L}^{(l)}_p$ \text{to} $\mathcal{L}_{\text{sens}}$
   
    % \State $W_k^{\text{grad}'} \leftarrow W_k^{\text{grad}} \oplus 2^{\text{MSB}}$ 
    %\State $L' \leftarrow \textit{BITFLIP}(\theta,W_{k}^{\text{grad}},B)$
    %\State $\Delta L_i^{\text{grad}} \leftarrow L' - L$
    %\State \text{Push} $\Delta L_i^{\text{grad}}$ \text{to} $L_{\text{hist}}$
    % \State \text{Revert changes}: $\theta' \leftarrow \theta$

    % \State $W_k^{\text{mix}'} \leftarrow W_k^{\text{mix}} \oplus 2^{\text{MSB}}$ 
    %\State $L' \leftarrow \textit{BITFLIP}(\theta,W_{k}^{\text{mix}},B)$
    %\State $\Delta L_i^{\text{mix}} \leftarrow L' - L$
    %\State \text{Push} $\Delta L_i^{\text{mix}}$ \text{to} $L_{\text{hist}}$
    % \State \text{Revert changes}: $\theta' \leftarrow \theta$
\EndFor    
    % \State \( R_{grad} \leftarrow \text{Layers ranked based on }  L_{\text{grad}}\)
    % \State \( R_{mag} \leftarrow \text{Layers ranked based on }  L_{\text{mag}}\)
\Ensure $\mathcal{L}_{\text{sens}}$%Layer rankings \( R_{grad}, R_{mag} \)
\end{algorithmic}
\label{alg:layer_ranking}
\end{algorithm}
% Algorithm \ref{alg:layer_ranking} delineates the layer ranking procedure, which begins by initializing two lists, \( L_{\text{mag}} \) and \( L_{\text{grad}} \), to store changes in the loss for weight magnitude and gradient perturbations, respectively (\textit{line 1}). For each layer \( i \) in the model, it selects the top-\( k \) weights based on their absolute magnitudes, denoted \( W_{\text{mag}}^k \) (\textit{line 3}), and gradients, denoted \( W_{\text{grad}}^k \) (\textit{line 4}). The selected weights are then perturbed by flipping the most significant bit (MSB) or negating them, resulting in \( W_{\text{mag}}^{k'} \) (\textit{line 5}). The model loss \( L' \) is computed after perturbation (line 6), and the change in the loss for magnitude perturbations, \( \Delta L_{\text{mag}}^i = L' - L \), is recorded in \( L_{\text{mag}} \) (\textit{lines 7-8}). The model parameters are reverted to their original state (line 9), and the same process is repeated for the gradient-based weights, updating \( W_{\text{grad}}^{k'} \) (line 10), calculating the new loss \( L' \) (\textit{line 11}), and recording \( \Delta L_{\text{grad}}^i \) in \( L_{\text{grad}} \) (\textit{lines 12-13}). After processing all layers, the layers are ranked based on the changes in loss from both \( L_{\text{grad}} \) and \( L_{\text{mag}} \) (\textit{lines 16-17}). Finally, the algorithm outputs the layer rankings \( R_{\text{grad}} \) and \( R_{\text{mag}} \).

%Algorithm \ref{alg:layer_ranking} outlines the layer ranking process by initializing lists \( L_{\text{mag}} \) and \( L_{\text{grad}} \) to store loss changes from magnitude and gradient perturbations, respectively (\textit{line 1}). For each layer \( i \), the top-\( k \) weights are selected based on absolute magnitudes \( W_{\text{mag}}^k \) (\textit{line 3}) and gradients \( W_{\text{grad}}^k \) (\textit{line 4}). These weights undergo perturbation by flipping the MSB or sign-bit to produce \( W_{\text{mag}}^{k'} \) (\textit{line 5}). The resulting model loss \( L' \) is computed, and the loss change \( \Delta L_{\text{mag}}^i = L' - L \) is recorded in \( L_{\text{mag}} \) (\textit{lines 6-8}). After reverting the parameters (\textit{line 9}), the same steps apply to gradient-based weights, updating \( W_{\text{grad}}^{k'} \) (\textit{line 10}), recalculating \( L' \) (line 11), and storing \( \Delta L_{\text{grad}}^i \) in \( L_{\text{grad}} \) (\textit{lines 12-13}). Layers are then ranked based on \( L_{\text{mag}} \) and \( L_{\text{grad}} \) (\textit{lines 16-17}). Finally, the algorithm outputs the layer rankings \( R_{\text{grad}} \) and \( R_{\text{mag}} \).



By iterating over layers and recording $\mathcal{L}_l$, we construct a corpus of bit-flip sensitivity metrics. This dataset enables the identification of the most sensitive layers in the model, thus guiding efficient allocation of analysis efforts toward layers where perturbations significantly degrade model performance.%Consequently, layers are ranked based on the resulting \(\Delta L\), yielding two distinct rankings: gradient-based ranking $R_{grad}$ and magnitude-based ranking $R_{mag}$.

Algorithm \ref{alg:layer_ranking} presents a systematic approach for conducting layer sensitivity analysis. The algorithm begins by initializing an empty set, $\mathcal{L}_{\text{sens}}$, designated to store the computed model loss resulting from parameter perturbations in each layer (\textit{line 1}).
The algorithm defines the function $\texttt{SSCORE}$, responsible for calculating sensitivity scores for each model parameter (\textit{lines 2-7}). Specifically, this function normalizes the weights and gradients to yield $\mathbf{W}_N$ and $\nabla \mathbf{W}_N$, respectively (\textit{lines 3-4}), and then computes the sensitivity scores $\mathbf{S}$ using Equation \ref{eq:sensitivity} (\textit{line 5}). Another function, $\texttt{BFLIP}$, is defined to calculate the model loss $\mathcal{L}$ when weight perturbations are applied to a specified layer (\textit{lines 8-17}). The function $\texttt{BFLIP}$ accepts as input the layer weight parameters $\mathbf{W}^{(l)}$, bit position $pos$ to be flipped, and perturbation indices $I$ (\textit{line 8}). It begins by storing a copy of the original weights $\mathbf{W}^{(l)}$ in $\mathbf{W}^{(l)}_{\text{orig}}$ for later restoration (\textit{line 9}). Then, it applies bit-flip perturbations to the weights $w_i^{(l)}$ at the specified indices $i \in I$ (\textit{lines 10-12}). The modified model, $\mathcal{M}$, is updated with the perturbed weights $\mathbf{W}^{(l)}$ via the $\texttt{UpdateModel}$ function (\textit{line 13}), after which the model loss corresponding to these perturbed weights is evaluated through $\texttt{ComputeLoss}$ (\textit{line 14}). To revert the perturbation, the function restores the model weights $\mathbf{W}^{(l)}$ to their original values $\mathbf{W}^{(l)}_{\text{orig}}$ (\textit{line 15}). Finally, the computed loss $\mathcal{L}$ is returned (\textit{line 16}).

The layer sensitivity analysis itself begins by iterating through each layer, assessing the model’s sensitivity to perturbations in each (\textit{lines 18-24}). First, the number of bits to be flipped, $k$, is calculated as a fraction of the total parameters in the layer, determined by $\texttt{cardinality}(\mathbf{W}^{(l)})$, multiplied by the sub-sampling rate $r$ (given as a percentage) and divided by 100 (\textit{line 19}). Sensitivity scores $\mathbf{S}^{(l)}$ for the weights in layer $l$ are then computed using the previously defined $\texttt{SSCORE}$ function (\textit{line 20}). Next, the $\texttt{Top-k}$ indices $I^{(l)}_{\text{hybrid}}$ are identified from $\mathbf{S}^{(l)}$ (\textit{line 21}). These indices, along with the weights $\mathbf{W}^{(l)}$ and bit position $pos$, are passed to the $\texttt{BFLIP}$ function to compute the perturbation-induced loss $\mathcal{L}^{(l)}_r$ (\textit{line 22}). The resulting loss $\mathcal{L}^{(l)}_r$ is then stored in $\mathcal{L}_{\text{sens}}$ (\textit{line 23}). This process continues until all layers have been processed, yielding the final sensitivity loss set $\mathcal{L}_{\text{sens}}$ as output (\textit{line 25}).


\subsubsection{Weight subset selection}\label{sec:subset_selection}

\begin{algorithm}[t]
\caption{Weight Subset Selection}
\begin{algorithmic}[1]
\Require $\mathbf{W}$, $\nabla \mathbf{W}$, $\alpha$, $\mathcal{L}_{sens}$, \text{sub-sampling rates }$\mathcal{R}$, \text{Loss threshold } $\mathcal{L}_{th}$, Number of top layers $n$
\State \text{Initialize sun-sampling loss:} $\mathcal{L}_{\text{sub}} = [\text{ }]$
\State $\mathcal{L}_{top} \gets \texttt{Top$n$}(\mathcal{L}_{sens})$
\ForAll{$l \in \mathcal{L}_{top}$}
\ForAll{$r \in \mathcal{R}$}
    \State $k \gets r*\texttt{cardinality}(\mathbf{W}^{(l)})/100$
    \State $\textbf{S}^{(l)}$$\gets$ \texttt{SScore}($|\mathbf{W}^{(l)}|$, $|\nabla \mathbf{W}^{(l)}|$, $\alpha$)
    \State $I^{(l)}_{\text{hybrid}} \gets \texttt{Top$k$Index}(\mathbf{S}^{(l)})$
    
    \State $\mathcal{L}^{(l)}_r \leftarrow \texttt{BFLIP}({\mathbf{W}^{(l)}, pos, I^{(l)}_{\text{hybrid}}})$
    \If{$\mathcal{L}^{(l)}_r \geq \mathcal{L}_{th}$} 
        \State \text{Push} $[l,\mathcal{L}^{(l)}_r,k,r]$ \text{to} $\mathcal{L}_{\text{sub}}$
        \State \textbf{break}
    \EndIf
    
\EndFor
\EndFor
\State $\mathcal{L}_{sub} \gets \texttt{SORT}(\mathcal{L}_{sub}) \text{ based on 3rd item }k$
\State $\mathcal{L}_{sub-1} \gets \mathcal{L}_{sub}[0]$
\State $l,k \gets \mathcal{L}_{sub-1}[0], \mathcal{L}_{sub-1}[2]$
\State $\textbf{S}^{(l)}$$\gets$ \texttt{SScore}($|\mathbf{W}^{(l)}|$, $|\nabla \mathbf{W}^{(l)}|$, $\alpha$)
\State $I^{(l)}_{\text{hybrid}} \gets \texttt{Top$k$Index}(\mathbf{S}^{(l)})$
\State $\mathcal{W}_{sub} \gets [l,I^{(l)}_{\text{hybrid}}]$
\Ensure $\mathcal{W}_{sub}$\Comment{Return weight subset}
\end{algorithmic}
\label{Algo:bitflip}
\end{algorithm}

\iffalse
\begin{algorithm}[t]
\caption{Weight Subset Selection}
\begin{algorithmic}[1]
\Require $\mathcal{L}_{sens}, \beta, n$
\Function{RankScore}{\text{row}, $\beta$}
    \State $N_{row} \gets \emph{row}[\text{number\_of\_weights\_flipped}]$
    \State $L_{row} \gets \emph{row}[\text{Model\_loss}]$
    \State $N_{max} \gets \emph{max}(\emph{row}[\text{number\_of\_weights\_flipped}])$
    \State $L_{max} \gets \emph{max}(\emph{row}[\text{Model\_loss}])$
    \State $L_{\text{norm}} \gets \frac{N_{row}}{N_{max}}$
    \State $W_{\text{norm}} \gets \frac{W_{row}}{W_{max}}$
    \State $\text{Score} \gets \beta \cdot L_{\text{norm}} - (1 - \beta) \cdot W_{\text{norm}}$
    \State \Return $\text{Score}$
\EndFunction
\For{each \emph{row} in $L_{hist}$}
    \State $\emph{row}[\text{Rank\_score}] \gets \emph{RankScore}(row, \beta)$
\EndFor
\State $L_{hist} \gets \emph{Sorted}
(L_{hist})$ \Comment{Sort based on \emph{Rank score}}
\State $W_s \gets \{w_i|i \in \text{weights in }L_{hist}[:n]\}$
\Ensure $W_s$\Comment{Return weight subset}
\end{algorithmic}
\label{Algo:bitflip}
\end{algorithm}
\fi

% Upon establishing the layer rankings from the layer sensitivity analysis performed in Section \ref{sec:layer_sensitivity}, we proceed to select an subset of model weights for identifying critical parameters. this subset selction is necessary to narrow down the critical weight space, which can be used for weight set optimization in the following section. The intuition behind it is that the larger the initial weight subset is, the less efficient will the optimization performance be due to the vastness of the solution space, hindering the convergence process.

% Towards this, we perform a similar weight perterbation experiment as done in SEction \ref{sec:layer_sensitivity} but only for $\texttt{Top}$n layers. We also vary the sub-sampling \% $p$ to observe at what value of $p$ does the perturbation loss $\mathcal{L}$ catches a predefined loss threshold $\mathcal{L}_{th}$, singnifying that further increment in $p$ is unnecessary for achiving critical modle performance degradation. We also keep track of the actual number of bit-flip perturbations $k$ along with $p$, which is later used for systematic selection of the weight-subspace. The need for storing $k$, is that due to layer \texttt{cardinality} variation, $k$ value can differ from layer to layer irrespective of same $p$. And this $k$ value is necessary to ensure that the smallest weight-subset is slected in this step.

% So for this weight subset selection, first we selct the $\texttt{Top-}n$ layers from the model leveraging the layer sensitivity infromation from Section \ref{sec:layer_sensitivity}. For each layer in the top-n, we vary the subasampling ratio from very low (0.0001\%) to a high value (10\%) in 10x increment and perform the weight perturbation experiment. as discussed in Section \ref{sec:layer_sensitivity}. for each of these experiment, the correspondig modle loss along with number of bit-flips $k$ is used to find the layer that achieves the target loss with minimum number of bit-flips. Finally that layer and the corresponding sub-sampled weight set is considered as the final weight subset for weight set optimization experimehts in the following sections.

Establishing layer rankings through sensitivity analysis in Section \ref{sec:layer_sensitivity} enables us to narrow down the subset of model weights required to identify critical parameters. By selecting a refined subset of weights, we can substantially limit the solution space for the weight-set optimization, improving computational efficiency and accelerating convergence. Without this reduction, the vast initial search space would hinder optimization performance.

To determine this subset, we conduct a perturbation experiment, similar to that in Section \ref{sec:layer_sensitivity}, but restricted to the top-\( n \) most sensitive layers. In this experiment, we vary the sub-sampling rate \( r \) across a defined range to identify the minimum \( r \) value at which the perturbation-induced loss \( \mathcal{L} \) reaches or exceeds a predefined threshold, \( \mathcal{L}_{\text{th}} \). This threshold represents a critical degradation in model performance, indicating that further increments in \( r \) are unnecessary. Recording the smallest \( r \) that meets \( \mathcal{L}_{\text{th}} \) achieves a balance between perturbation efficacy and computational expense.

For each selected layer, the bit-flip count \( k \) is calculated to correspond to the layer’s weight cardinality and the sub-sampling ratio \( p \) using Equation \ref{eq:topk}. 
This count ensures that variations in layer sizes are accommodated, with larger layers naturally requiring more bit-flips to induce equivalent perturbations. By recording both \( k \) and \( r \) for each top layer, we can identify the smallest set of weights in each layer that achieves the target loss, enabling efficient subset selection.

Once each layer has been assessed for optimal sub-sampling values, we determine the specific layer \( l \) and corresponding values of \( k \) and \( r \) that yield the smallest subset satisfying the threshold condition \( \mathcal{L} \geq \mathcal{L}_{\text{th}} \). The resulting subset configuration represents the most efficient collection of weights for further refinement. Defining the critical weight subset \( \mathcal{W}_{\text{sub}} \) as:
\begin{equation}
    \mathcal{W}_{\text{sub}} = \{\mathbf{W}^{(l)}_i \mid i \in I^{(l)}_{\text{hybrid}}, |I^{(l)}_{\text{hybrid}}| = k\},
\end{equation}

we obtain a minimal yet impactful subset of weights, ensuring optimized computational performance in weight-set optimization in subsequent sections. This approach strategically minimizes the complexity of future stages while preserving the effectiveness of targeted parameter refinement.

The weight subset selection procedure, outlined in Algorithm \ref{Algo:bitflip}, takes as inputs the model weights \(\mathbf{W}\), gradients \(\nabla \mathbf{W}\), sensitivity ratio \(\alpha\), layer sensitivity \(\mathcal{L}_{\text{sens}}\), sub-sampling rates \(\mathcal{R}\), a loss threshold \(\mathcal{L}_{\text{th}}\), and the number of top layers \(n\), and outputs a weight subset \(\mathcal{W}_{\text{sub}}\).

The process begins with initializing a list, \(\mathcal{L}_{\text{sub}}\), to record losses (\textit{line 1}). The top \(n\) layers are selected based on \(\mathcal{L}_{\text{sens}}\), following the model loss computation detailed in Section \ref{sec:layer_sensitivity} (\textit{line 2}). For each of these top layers, the algorithm iterates through sub-sampling ratios \(p\), computing the perturbation loss induced by bit flips (\textit{lines 3-14}). Specifically, the number of bits to flip, \(k\), is computed as a fraction of the total parameters in the layer using Equation \ref{eq:topk} (\textit{line 5}). Sensitivity scores \(\mathbf{S}^{(l)}\) are then calculated for layer \(l\) using the \texttt{SSCORE} function (\textit{line 6}), and the indices \(I^{(l)}_{\text{hybrid}}\) of the \texttt{Top-k} scores are identified (\textit{line 7}). These indices, along with the corresponding weights \(\mathbf{W}^{(l)}\) and a specified bit position \(pos\), are input to the \texttt{BFLIP} function, which returns the perturbation loss \(\mathcal{L}^{(l)}_r\) (\textit{line 8}).

If \(\mathcal{L}^{(l)}_r \geq \mathcal{L}_{\text{th}}\), this loss, along with layer index \(l\), \(k\), and \(r\), is stored in \(\mathcal{L}_{\text{sub}}\), and further iterations for that layer are halted (\textit{lines 9-12}); otherwise, iterations continue until \(\mathcal{R}\) is exhausted. After completing this sub-sampling procedure, the loss data in \(\mathcal{L}_{\text{sub}}\) is sorted by \(k\) (\textit{line 15}), yielding an ordered set where the smallest weight subset achieving the target loss is prioritized. The layer \(l\) and subset size \(k\) for this smallest subset are then extracted (\textit{lines 16-17}). Sensitivity scores \(\mathbf{S}^{(l)}\) are recalculated for layer \(l\) (\textit{line 18}), and the indices \(I^{(l)}_{\text{hybrid}}\) corresponding to the \texttt{Top-k} scores are selected (\textit{line 19}). Finally, the identified subset \(\mathcal{W}_{\text{sub}}\) for layer \(l\) and \(I^{(l)}_{\text{hybrid}}\) is returned as the algorithm's output.
\iffalse
The weight subset selection process is formalized in Algorithm \ref{Algo:bitflip}, which takes as inputs the model weights, \(\mathbf{W}\), gradients, \(\nabla\mathbf{W}\), sensitivity ratio \(\alpha\), layer sensitivity, \(\mathcal{L}_{\text{sens}}\), sub-sampling rates, \(\mathcal{P}\), a loss threshold, \(\mathcal{L}_{\text{th}}\), and the number of top layers, \(n\). The algorithm outputs a subset of weights, \(\mathcal{W}_{\text{sub}}\), optimized for targeted model bit-flip attack.

The algorithm starts by initializing an empty list, \(\mathcal{L}_{\text{sub}}\), to store results for perturbation-based loss experiments (\textit{line 1}). The \(\texttt{Top-}n\) layers are selected from \(\mathcal{L}_{\text{sens}}\) (\textit{line 2}). For each layer \(l\) among these top layers, the sub-sampling rates \(p\) are iteratively tested, with the corresponding perturbation-induced model loss calculated for each rate (\textit{lines 3-14}).

Specifically, for each layer, the number of bits to be flipped, \(k\), is determined as $k = \texttt{cardinality}(\mathbf{W}^{(l)})*p/100$,
where \(\texttt{cardinality}(\mathbf{W}^{(l)})\) represents the total parameters in layer \(l\) (\textit{line 5}). Subsequently, the sensitivity scores, \(\mathbf{S}^{(l)}\), for weights within layer \(l\) are computed by invoking the \(\texttt{SSCORE}\) function (\textit{line 6}). Based on these scores, the \(\texttt{Top-k}\) indices, \(I^{(l)}_{\text{hybrid}}\), are identified from \(\mathbf{S}^{(l)}\) (\textit{line 7}). The selected indices, weights \(\mathbf{W}^{(l)}\), and bit position \(pos\) are then provided as input to the \(\texttt{BFLIP}\) function, which computes the perturbation-induced loss, \(\mathcal{L}^{(l)}_p\) (\textit{line 8}).

This loss, \(\mathcal{L}^{(l)}_p\), is subsequently compared to the threshold \(\mathcal{L}_{\text{th}}\). If \(\mathcal{L}^{(l)}_p \geq \mathcal{L}_{\text{th}}\), the results—including the layer index \(l\), bit-flip count \(k\), and subsampling rate \(p\)—are stored in \(\mathcal{L}_{\text{sub}}\), and the iteration for that layer terminates (\textit{lines 9-12}). Otherwise, the algorithm continues until all values of \(\mathcal{P}\) are exhausted.
Upon completing this layer-wise subsampling and perturbation process, the loss list \(\mathcal{L}_{\text{sub}}\) is sorted by the parameter \(k\), resulting in a prioritized list where the smallest subset of weights causing substantial loss appears first (\textit{line 15}). The first layer $\mathcal{L}_{\text{sub-1}}$ is then selected from \(\mathcal{L}_{\text{sub}}\)for weight subset creation (\textit{line 16}).

The corresponding layer \(l\) and bit-flip count \(k\) values are extracted from \(\mathcal{L}_{\text{sub-1}}\) list (\textit{line 17}). Using these values, the sensitivity scores, \(\mathbf{S}^{(l)}\), are recalculated (\textit{line 18}), and the \(\texttt{Top-k}\) indices, \(I^{(l)}_{\text{hybrid}}\), representing the most sensitive weights in layer \(l\), are selected (\textit{line 19}). Finally, the selected indices \(I^{(l)}_{\text{hybrid}}\) in layer \(l\) are used to form the weight subset \(\mathcal{W}_{\text{sub}}\), which serves as the algorithm’s output.

% The procedure for weight subset selection is outlined in Algorithm \ref{Algo:bitflip}, which takes the model weights $\mathbf{W}$, gradients $\nabla\mathbf{W}$,  sensitivity ratio $\alpha$, layer sensitivity $\mathcal(L)_{sens}$, sub-smapling rates $\mathcal{P}$, loss threshold $\mathcal(L)_{th}$ and number of top layers $n$ as inputs and provides a weight subset $\mathcal{W}_{sub}$ as output. It begins by initializing a loss list $\mathcal{L}_{sub}$ (\textit{line 1}). Now the $\texttt{Top}n$ layers are chosen from $\mathcal(L)_{sens}$ using the model loss calculated in section \ref{sec:layer_sensitivity} (\textit{line 2}). Then for each layer in $\texttt{Top}n$ layers, the sub-sampling ratios $p$s are varied and the corrsponding model pertabation loss is evaluated (\textit{lines 3-14}). For this,  First, the number of bits to be flipped, $k$, is calculated as a fraction of the total parameters in the layer, determined by $\texttt{cardinality}(\mathbf{W}^{(l)})$, multiplied by the sub-sampling rate $p$ (given as a percentage) and divided by 100 (\textit{line 5}). Sensitivity scores $\mathbf{S}^{(l)}$ for the weights in layer $l$ are then computed using the previously defined $\texttt{SSCORE}$ function (\textit{line 6}). Next, the $\texttt{Top-k}$ indices $I^{(l)}_{\text{hybrid}}$ are identified from $\mathbf{S}^{(l)}$ (\textit{line 7}). These indices, along with the weights $\mathbf{W}^{(l)}$ and bit position $pos$, are passed to the $\texttt{BFLIP}$ function to compute the perturbation-induced loss $\mathcal{L}^{(l)}_p$ (\textit{line 8}). The resulting loss $\mathcal{L}^{(l)}_p$ is then compared against the loss threshold c, which if greater or equal to $\mathcal(L)_{th}$ is stored in $\mathcal{L}_{sub}$ along with layer index $l$, $k$ and $p$ and the iteration for that layer is terminated (\textit{lines 9-12}). Else the iteration is continued untill $\mathcal{P}$ exhausts. Upon completion of this layer wise sub-sampling based model perturbation experiment, we $\texttt{SORT}$ the loss corpus $\mathcal{L}_{sub}$ based on the 3rd element ($k$) if each data point (\textit{line 15}), which results in an ordered $\mathcal{L}_{sub}$ with the smallest weight subset information being the first datapoint. Following which, the select the best layer to get the smallest subset of weights achiveing target loss $\mathcal{L}_{sub}$ (\textit{line 16}). The layer $l$ and $k$ values are then extracted from  $\mathcal{L}_{sub}$ (\textit{line 17} and used to calculate the sensitivity scores $\mathbf{S}^{(l)}$ (\textit{line 18} and the respective $\texttt{Top}k$ highest sensitive weights index selection (\textit{line 19}. The layer $l$ and its indexes $I^{(l)}_{\text{hybrid}}$ are then used to form the weight subset $\mathcal{W}_{sub}$, which is provided as output from the algorithm.

%Upon establishing the layer rankings, we proceed to refine the solution space for critical weights by selecting a subset based on the bit-flip sensitivity metrics, \( L_{\text{hist}} \), evaluated using Algorithm \ref{alg:layer_ranking}. To facilitate the subsequent optimization phase, we define a rank score function that quantifies the importance of each weight parameter. The rank score denoted as \( S(w_i) \), is a function of two key factors: the model loss, \( L_i \), induced by perturbing the weight \( w_i \), and the number of weights, \( N_i \), involved in achieving this perturbation. Intuitively, the rank score should increase with a higher model loss, \( L_i \), indicating a more impactful perturbation, while it should reduce as the number of weights, \( N_i \), decreases, reflecting the desirability of minimal perturbations. To balance these competing influences, we introduce a weightage parameter \( \beta \in [0, 1] \), which determines the relative importance of model loss and weight perturbation. The rank score function is then expressed as:

% \begin{equation}
%     S(w_i) = \beta \cdot L_i + (1 - \beta) \cdot N_i
% \end{equation}

%where \( L_i \) represents the model loss due to perturbing the weight \( w_i \), \( N_i \) denotes the number of weights perturbed to achieve the given loss, and \( \beta \) is the parameter that governs the trade-off between these two factors. The parameter \( \beta \) is selected to optimally balance the effect of model loss and weight perturbations, ensuring that the rank score reflects both the magnitude of the loss and the efficiency of the perturbation. Following the computation of rank scores for all weights in the set \( L_{\text{hist}} \), the weights are ranked in descending order. The top \( n \) layers, corresponding to the highest rank scores, are selected to create the critical weight subspace \( W_{\text{critical}} \), which encompasses the weights that exert the most significant influence on model performance with minimal perturbations. This critical weight subspace is subsequently utilized in the next optimization phase, ensuring both efficacy and efficiency in further model manipulation.


% Algorithm \ref{Algo:bitflip} describes the weight subset selection procedure, which begins by defining a ranking function, `RANKSCORE', to calculate a score for each row in \( L_{\text{hist}} \) based on the model’s loss and number of weights flipped (\textit{line 1}). For each row, it first extracts the number of weights flipped, \( N_{\text{row}} \), and the model loss, \( L_{\text{row}} \) (\textit{lines 2-3}). The function also computes maximum values \( N_{\text{max}} \) and \( L_{\text{max}} \) from these respective columns (\textit{lines 4-5}). Using these, it normalizes \( L_{\text{row}} \) and \( N_{\text{row}} \) to \( L_{\text{norm}} \) and \( W_{\text{norm}} \) (\textit{lines 6-7}). The final ranking score is calculated as \( \text{Score} = \beta \cdot L_{\text{norm}} - (1 - \beta) \cdot W_{\text{norm}} \), balancing model loss and the weight subset size by the parameter \( \beta \) (\textit{line 8}). The function returns this score (line 9). Next, for each row in \( L_{\text{hist}} \), the `RANKSCORE' function is used to assign a rank score (\textit{lines 11-13}). The algorithm sorts \( L_{\text{hist}} \) in descending order by the rank score (\textit{line 14}). Finally, the top \( n \) weights are selected, forming \( W_s \), and are returned as the optimal weight subset (\textit{line 15}).


After establishing layer rankings, we refine the solution space for critical weights by selecting and evaluating a subset of weights using a systematic perturbation experiment. 

Let \(\{L_{\text{top-n}}^{\text{grad}}, L_{\text{top-n}}^{\text{mag}}\}\) represent the top-\(n\) layers identified by gradient-based ranking \(R_{\text{grad}}\) and magnitude-based ranking \(R_{\text{mag}}\), respectively. For each layer \(l \in L_{\text{top-n}}^{\text{grad}} \cup L_{\text{top-n}}^{\text{mag}}\), we select the top-\(k\) weights \(\{w_i\}_{i=1}^k\) and compute their sensitivity scores \(S(w_i)\) by varying the parameter \(\alpha \in [0,1]\) as follows:
\begin{equation}
    S(w_i) = \alpha \cdot |\nabla L(w_i)| + (1 - \alpha) \cdot |w_i|
\end{equation}

where \(\alpha = 0\) emphasizes weight magnitudes \(|w_i|\), \(\alpha = 1\) emphasizes gradients \(|\nabla L(w_i)|\), and intermediate values adjust the balance. For each \(w_i\), this scoring function \(S(w_i)\) thus quantifies sensitivity by weighting both the parameter’s magnitude and gradient information.

The weights are collated and sorted in descending order of \(S(w_i)\), yielding a prioritized list of the most critical weights in the selected layers. Starting with the highest-ranked weights, we iteratively perturb each \(w_i\) by flipping the most significant bit (MSB) or the sign bit, yielding a perturbed weight \(w_i'\).

After each perturbation, we compute the updated model loss, \(L'\), and calculate the cumulative change in loss. This process continues, with each subsequent perturbation contributing to \(\Delta L\), until the cumulative model loss exceeds a predefined threshold \(L_{\text{threshold}}\), indicating a boundary for effective model performance. At this threshold, we define the \textbf{weight subspace} \(\mathcal{W}_{\text{critical}}\) as the subset of perturbed weights \(\{w_i' \in \mathcal{W}_{\text{top-k}}\}\) that were altered to reach \(L_{\text{threshold}}\):
\begin{equation}
    \mathcal{W}_{\text{critical}} = \{w_i' \mid \Delta L \geq L_{\text{threshold}}\}
\end{equation}

The set \(\mathcal{W}_{\text{critical}}\) constitutes the critical weight subspace, representing a reduced solution space of parameters with the most significant impact on model robustness.
 

Algorithm \ref{Algo:bitflip} defines a systematic BFA on model parameters, consisting of three main functions. The SSCORE function (\textit{lines 1-6}) takes weights, gradients, and a sensitivity parameter \(\alpha\) as inputs. It normalizes the weights and gradients, denoted as \(W_{\text{norm}}\) and \(G_{\text{norm}}\) respectively (\textit{lines 2-3}), and computes a sensitivity score by combining them using \(\alpha\)(\textit{line 4}). The COLLATE function (\textit{lines 7-17}) then aggregates parameters across layers, initializing an empty parameter storage list (\textit{line 8}). For each layer \(l\) (\textit{line 9}), it retrieves the layer’s weights and gradients (lines 10-11), computes sensitivity scores using the SSCORE function (\textit{line 12}), and selects the top-\(k\) parameters based on these scores (\(S_k\), \textit{line 13}). It appends the resulting weight and score pairs \((W_k, S_k)\) to the parameter list (\textit{line 14}). Finally, the BITFLIP function (\textit{lines 18-24}) conducts the attack by selecting the top-\(k\) parameters from the collated list (\textit{line 19}) and iteratively applying bit-flips at each position \(B\) to the selected parameters using the XOR operation \(\theta_{l,i} \oplus (1 \ll B)\) (\textit{line 21}). This operation updates each \(\theta_{l,i}\) in \(W_k\) and concludes the attack.
\fi



\subsubsection{Weight-set optimization}\label{sec:genetic}
After identifying the weight subspace \(\mathcal{W}_{\text{sub}}\), further refinement is essential given that LLMs typically encompass billions of parameters and tens of billions of bits. Consequently, a crude attack targeting thousands or even millions of parameters—implying tens of millions of bit-flips—would be prohibitive from an attacker's perspective due to resource intensiveness. Therefore to address this issue, for optimizing BFA, we systematically reduce \(\mathcal{W}_{\text{sub}}\) to $\mathcal{W}_S$ ($\mathcal{W}_S \subset \mathcal{W}_{\text{sub}}$) by isolating a smaller subset of parameters capable of achieving comparable degradation in model performance.
%Given the nonlinear relationship inherent in determining this subset, gradient-free optimization methods are suitable. These techniques allow us to effectively navigate the search space without relying on gradient information. 
To this end, we design a novel algorithm inspired by evolutionary and genetic strategies, formulated specifically to identify a minimal, highly impactful subset of critical weights, thereby optimizing the impact-to-size ratio of the targeted parameters for BFA.  

%Here, We define how we develop the algorithm for convergence toward an optimal subset of critical weights, \(\mathcal{W}_{\text{opt}}\), under the specified constraints.

\noindent\textbf{Objective Function and Fitness Evaluation:}
Given the initial weight subset \(\mathcal{W}_{\text{sub}} = \{ w_1, w_2, \ldots, w_N \}\) and target model loss threshold \(\mathcal{L}_{\text{th}}\), the goal is to identify a weight subset \(\mathcal{W}_{S_j} \subset \mathcal{W}_{\text{sub}}\) such that bit-flipping this subset maximizes the model loss while reducing the set size or \texttt{cardinality}, which signifies the number of bit-flips to get the corresponding model loss. We define each solution \(\mathcal{W}_{S_j} = \{ w_{j_1}, w_{j_2}, \ldots \}\) as a candidate subset weights.
For each solution \(\mathcal{W}_{S_j}\), the fitness function \(f(\mathcal{W}_{S_j})\) is computed by,
\begin{equation}
    f(\mathcal{W}_{S_j}) = \frac{\mathcal{L}_{S_j}}{\texttt{cardinality}(\mathcal{W}_{S_j})}
\end{equation}
where $\mathcal{L}_{S_j}$ represents the model loss after bit-flipping all weights in \(\mathcal{W}_{S_j}\). Thus, the problem is formulated as maximization of model loss while minimizing \texttt{cardinality}, equivalent to maximizing the fitness function.

\noindent\textbf{Population Initialization:}
A population $\mathbf{P}$ is defined with \(m\) solutions as \(\mathbf{P} = \{ \mathcal{W}_{S_1}, \mathcal{W}_{S_2}, \ldots, \mathcal{W}_{S_m} \}\). 
The first solution $\mathbf{P}_0$ is initialized as the initial weight subset $\mathcal{W}_{\text{sub}}$, then each new solution $\mathbf{P}_j$ is formed by mutating $\mathbf{P}_0$. 

\begin{equation}
    \mathbf{P}_j \gets \texttt{Mutate}(\mathbf{P}_0)
\end{equation}

This \textbf{Mutation} operation is defined as follows:

\noindent\textbf{Mutation Operation:}
In \textbf{Mutation} operation each solution undergoes mutation at a rate \(\mu\), modifying the solution by removing some weights by replacing them with new weights from \(\mathcal{W}_{\text{sub}}\). Formally, for each weight \(w_{j_i} \in \mathbf{P}_{oj}\), with probability \(\mu\), we replace \(w_{j_i}\) with a randomly selected \(w_k \in \mathcal{W}_{\text{sub}}\):
\begin{equation}
    w_{j_i}' = \begin{cases} 
      w_k, & \text{with probability } \mu \\
      w_{j_i}, & \text{otherwise}.
   \end{cases}
\end{equation}

Mutation introduces diversity, ensuring the algorithm explores a broader solution space.

%Each solution \(\mathcal{W}_{S_j}\) or $\mathbf{P}_{j}$ is initialized by selecting \(n\) weights randomly from \(\mathcal{W}_{\text{sub}}\) (\textit{i.e.}, \(\texttt{cardinality}(\mathcal{W}_{S_j}) = n\) and \(\mathcal{W}_{S_j} \subset \mathcal{W}_{\text{sub}}\)).

\noindent\textbf{Elitism and Selection:}
At each generation \(t\), all solutions in \(\mathbf{P}\) are sorted by their fitness values:
\begin{equation}
    \mathbf{P}_{\text{best}} = \mathcal{W}_{S_{\text{best}}} = \arg \min_{\mathbf{P}_{j} \in \mathbf{P}} f(\mathbf{P}_{j})
\end{equation}
where \(\mathcal{W}_{S_{\text{best}}}\) or $\mathbf{P}_{best}$ represents the solution with the highest fitness (\textit{i.e.}, most effective in degrading model performance). Elitism dictates that $\mathbf{P}_{j}$ is carried forward unchanged into the next generation, ensuring the highest-quality solution is preserved.
For the remaining solutions, a tournament selection strategy is employed to choose pairs of solutions for crossover, which involves choosing two random solutions \(\mathbf{P}_{a}, \mathbf{P}_{b} \in \mathbf{P}\), and selecting the one with better fitness:
\begin{equation}
    \mathbf{P}_{p} = \arg \min \{ f(\mathbf{P}_{a}), f(\mathbf{P}_{ b}) \}.
\end{equation}
\noindent\textbf{Crossover Operation:}
To produce new solutions, two-parent solutions, \( \mathbf{P}_{p1} \) and \( \mathbf{P}_{2} \), are selected, and a crossover operation is performed with probability \( p_c \). For each gene \( g_i \) in the parent solutions, a stochastic decision determines whether \( g_i \) from \( \mathbf{P}_{p1} \) and \( \mathbf{P}_{p2} \) is incorporated into the offspring. This procedure yields two offspring, \( \mathbf{P}_{o1} \) and \( \mathbf{P}_{o2} \), formed by combining genes from both parents:
\begin{equation}
    \mathbf{P}_{o1} = \{g_i^{\mathbf{P}_{p1}} \text{ or } g_i^{\mathbf{P}_{p2}}\} \quad \forall i
\end{equation}
\begin{equation}
    \mathbf{P}_{o2} = \{g_i^{\mathbf{P}_{p2}} \text{ or } g_i^{\mathbf{P}_{p1}}\} \quad \forall i
\end{equation}
If no crossover occurs (\textit{i.e.}, with probability \( 1 - p_c \)), the offspring remain identical to the parents: \( \mathbf{P}_{o1} = \mathbf{P}_{p1} \) and \( \mathbf{P}_{o2} = \mathbf{P}_{p2} \). This preserves beneficial traits from both parents while maintaining genetic diversity in the offspring.
% \subsubsection{Crossover Operation}

% To generate new solutions, two-parent solutions, \(P_1\) and \(P_2\), are selected. A crossover point \(c\) is chosen randomly along the solution, and offspring \(O_1\) and \(O_2\) are generated by swapping portions of the parent solutions:
% \[
% O_1 = \{ P_1[:c] \cup P_2[c:] \}, \quad O_2 = \{ P_2[:c] \cup P_1[c:] \}.
% \]

% These offspring solutions ensure a recombination of weights, preserving advantageous characteristics from both parents while introducing variation.



\noindent\textbf{Convergence and Termination:}
This process continues over generations \(t = 1, 2, \ldots, g\), where \(g\) is the maximum iteration count (pre-defined). The algorithm terminates if either the target model loss is achieved ($ \mathcal{L}_{\mathbf{P}_{\text{best}}} \leq \mathcal{L}_{\text{th}}$) or the iteration limit \(g\) is reached ($t == g$).
The final output is the subset \(\mathcal{W}_{\text{opt}} \subset \mathcal{W}_{\text{sub}}\), where 
\begin{equation}
    \mathcal{W}_{\text{opt}} = \arg \min_{\mathbf{P}_{j} \in \mathbf{P}} f(\mathbf{P}_{j})
\end{equation}
representing the critical weights necessary to achieve the targeted model loss degradation. This subset not only reduces the solution space for adversarial interventions but also provides a computationally optimal and diverse set of weight parameters. The iterative refinement ensures the proposed approach explores and exploits the search space, optimizing both the quality and variety of solutions.

\begin{algorithm}[t]
\caption{Weight Set Optimization}
\begin{algorithmic}[1]
\Require $\mathbf{W}$, Weight subset $\mathbf{W}_{\text{sub}}$, Target loss threshold $\mathcal{L}_{\text{th}}$, solution size $n$, population size $m$, max generations $g$, mutation/reduction rate $\mu$
% \Ensure Optimized weight subset $\mathcal{W}_{\text{opt}}$
\State \text{Initialize solution space }$\mathbf{SS} = [\text{ }], \text{ solution set }\mathbf{P} = [\text{ }], \text{ fitness score list } \mathbf{F} = [\text{ }]$
\State $l,\mathbf{SS} \gets \mathbf{W}_{\text{sub}}[0], \mathbf{W}_{\text{sub}}[1]$
\State $\mathbf{P}_0 \gets [\mathbf{SS}]$
\State $\text{Push } \mathbf{P}_0 \text{ to } \mathbf{P}$
\For{$j = 1,2,...,m$}\Comment{Initialize population}
\State $\mathbf{P}_j \gets \texttt{Mutate}(\mathbf{P}_0)$
\State $\text{Push } \mathbf{P}_j \text{ to } \mathbf{P}$
\EndFor
% \State $\mathcal{P} \gets$ \Call{InitializePopulation}{$\mathcal{W}_{\text{critical}}, n, m$} 
\For{$t = 1, 2, \dots, g$}
\For{$j = 1,2,...,m$}
\State $\mathbf{W}^{(l)} = \texttt{GetParams}(\mathbf{W},l)$
\State $I^{(l)}_{\text{hybrid}} \gets \mathbf{P}_{j}$
    \State $f \leftarrow \texttt{BFLIP}
    ({\mathbf{W}^{(l)}, pos, I^{(l)}_{\text{hybrid}}})$
    
\State \text{Push} $f$ \text{to} $\mathbf{F}$
\EndFor
    \State $\mathbf{P} \gets \texttt{SortSolutions}({\mathbf{P},\mathbf{F}})$ 
    \State $\mathbf{P}_{best} \gets$ \texttt{SelectBestSolution}({$\mathbf{P}$}) 
    % \State $f_{\text{best}} \gets$ \texttt{SelectBestFitness}({$\mathbf{F}$}) 
    \State $\mathbf{P}_{\text{new}} \gets [\mathbf{P}_{\text{best}},\texttt{Mutate}(\mathbf{P}_{best})]$ 
    \While{$\texttt{len}(\mathbf{P}_{\text{new}}) < m$}
        \State $\mathbf{P}_{p1}, \mathbf{P}_{p2} \gets$ \texttt{TournamentSelection}($\mathbf{P},\mathbf{F}$)
        \State $\mathbf{P}_{o1}, \mathbf{P}_{o2} \gets$ \texttt{Crossover}($\mathbf{P}_{best},\mathbf{P}_{p1}, \mathbf{P}_{p2}$)
        \State $\mathbf{P}_{o1}, \mathbf{P}_{o2} \gets$ \texttt{Mutate}{($\mathbf{P}_{o1}, \mathbf{P}_{o2}, \mu$)} 
        \State Push $\mathbf{P}_{o1}$ and $\mathbf{P}_{o2}$ to $\mathbf{P}_{\text{new}}$
    \EndWhile
    \State $\mathbf{P} \gets \mathbf{P}_{\text{new}}$ \Comment{Population for next generation}
\EndFor
\Ensure $\mathbf{P}_{\text{best}}$ \Comment{Return best solution}
\end{algorithmic}
\label{algo:genetic}
\end{algorithm}

\iffalse
\begin{algorithm}[t]
\caption{Weight Set Optimization}
\begin{algorithmic}[1]
\Require $\mathbf{W}$, Weight subset $\mathbf{W}_{\text{sub}}$, Target loss threshold $\mathcal{L}_{\text{th}}$, solution size $n$, population size $m$, max generations $g$, mutation/reduction rate $\mu$
% \Ensure Optimized weight subset $\mathcal{W}_{\text{opt}}$
\State \text{Initialize solution space }$\mathbf{SS} = [\text{ }], \text{ solution set }\mathbf{P} = [\text{ }], \text{ fitness score list } \mathbf{F} = [\text{ }]$
\State $l,\mathbf{SS} \gets \mathbf{W}_{\text{sub}}[0], \mathbf{W}_{\text{sub}}[1]$
\For{$j = 1,2,...,m$}\Comment{Initialize population}
\State $\mathcal{W}_{S_j} \gets \texttt{random.sample}(\mathbf{SS},n)$
\State $\text{Push } \mathcal{W}_{S_j} \text{ to } \mathbf{P}$
\EndFor
% \State $\mathcal{P} \gets$ \Call{InitializePopulation}{$\mathcal{W}_{\text{critical}}, n, m$} 
\For{$t = 1, 2, \dots, g$}
\For{$j = 1,2,...,m$}
\State $\mathbf{W}^{(l)} = \texttt{GetParams}(\mathbf{W},l)$
\State $I^{(l)}_{\text{hybrid}} \gets \mathbf{P}_{j}$
    \State $f \leftarrow \texttt{BFLIP}
    ({\mathbf{W}^{(l)}, pos, I^{(l)}_{\text{hybrid}}})$
    
\State \text{Push} $f$ \text{to} $\mathbf{F}$
\If{$f \geq \mathcal{L}_{\text{th}}$} 
        \State \Return $\mathbf{P}_{j}$ 
    \EndIf
\EndFor
    \State $\mathbf{P} \gets \texttt{SortSolutions}({\mathbf{P},\mathbf{F}})$ 
    \State $\mathbf{P}_{best} \gets$ \texttt{SelectBestSolution}({$\mathbf{P}$}) 
    % \State $f_{\text{best}} \gets$ \texttt{SelectBestFitness}({$\mathbf{F}$}) 
    \State $\mathbf{P}_{\text{new}} \gets [\mathbf{P}_{\text{best}}]$ 
    \While{$\texttt{len}(\mathbf{P}_{\text{new}}) < m$}
        \State $\mathbf{P}_{p1}, \mathbf{P}_{p2} \gets$ \texttt{TournamentSelection}($\mathbf{P},\mathbf{F}$)
        \State $\mathbf{P}_{o1}, \mathbf{P}_{o2} \gets$ \texttt{Crossover}($\mathbf{P}_{p1}, \mathbf{P}_{p2}$)
        \State $\mathbf{P}_{o1}, \mathbf{P}_{o2} \gets$ \texttt{Mutate}{($\mathbf{P}_{o1}, \mathbf{P}_{o2}, \mu, \mathbf{SS}$)} 
        \State Push $\mathbf{P}_{o1}$ and $\mathbf{P}_{o2}$ to $\mathbf{P}_{\text{new}}$
    \EndWhile
    \State $\mathbf{P} \gets \mathbf{P}_{\text{new}}$ \Comment{Population for next generation}
\EndFor
\Ensure $\mathbf{P}_{\text{best}}$ \Comment{Return best solution}
\end{algorithmic}
\label{algo:genetic}
\end{algorithm}
\fi
% Algorithm \ref{algo:genetic} describes the genetic optimization for reducing the critical weight subset, refining the initial weight set \(\mathbf{W}_{\text{sub}}\) generated in Algorithm \ref{Algo:bitflip} to meet a specific loss threshold \(\mathcal{L}_{\text{th}}\). Inputs include the model weights \(\mathbf{W}\), critical subset \(\mathbf{W}_{\text{sub}}\), threshold \(\mathcal{L}_{\text{th}}\), parameters for subset size \(n\), population size \(m\), maximum iterations \(g\), crossover probability \(p_c\), and mutation rate \(\mu\). 

% The algorithm first initializes empty lists for solution space \(\mathbf{SS}\), population \(\mathbf{P}\), and fitness scores \(\mathbf{F}\) (\textit{line 1}). It then extracts the target layer \(l\) and weight indices from \(\mathbf{W}_{\text{sub}}\) to define the initial solution space (\textit{line 2}). Using random sampling, \(m\) initial solutions are generated in \(\mathbf{P}\) (\textit{lines 3-5}). 

% For each iteration in the genetic loop, the algorithm evaluates each solution by applying selected weights \(\mathbf{W}^{(l)}\) and indices \(I^{(l)}_{\text{hybrid}}\) from \(\mathbf{P}\) to the \texttt{BFLIP} function, generating the corresponding model loss as a fitness score \(f\) (\textit{lines 9-12}). If any solution’s \(f \geq \mathcal{L}_{\text{th}}\), the algorithm terminates, returning that solution (\textit{lines 13-15}). If not, the process continues up to \(g\) iterations.

% Within each iteration, solutions are ranked in descending order by fitness scores \(\mathbf{F}\) (\textit{line 17}), with the best solution \(\mathbf{P}_{\text{best}}\) selected and included in the new population \(\mathbf{P}_{\text{new}}\) to preserve elitism (\textit{lines 18-19}). For remaining solutions, pairs of parents are chosen through tournament selection (\textit{line 21}), and each pair undergoes crossover to produce two offspring (\textit{line 22}), followed by mutation with probability \(\mu\) (\textit{line 23}). Offspring are added to \(\mathbf{P}_{\text{new}}\) until it reaches size \(m\) (\textit{line 24}).

The optimization algorithm (Algorithm \ref{algo:genetic}) employs an evolutionary strategy to refine a weight subset, \(\mathcal{W}_{sub}\), from Algorithm \ref{Algo:bitflip}. The algorithm receives model weights \(\mathcal{W}\), the targeted loss threshold \(\mathcal{L}_{\text{th}}\), and parameters for population characteristics: weight indices per candidate \(n\), population size \(m\), maximum iterations \(g\), crossover probability \(p_c\), and mutation rate \(\mu\). 

Initially, the algorithm sets up empty lists for the solution space \(\mathbf{SS}\), population \(\mathbf{P}\), and fitness scores \(\mathbf{F}\) (\textit{line 1}). The attacked layer \(l\) and initial solution space are derived from \(\mathcal{W}_{sub}\) (line 2). A population of \(m\) solutions is generated through random sampling and stored in \(\mathbf{P}\) (\textit{lines 3-5}). 

For each iteration \(t = 1, \dots, g\), the algorithm evaluates solutions by applying the \texttt{BFLIP} function on each weight subset \(\mathbf{W}^{(l)}\) and indices \(I^{(l)}_{\text{hybrid}}\), producing a model loss \(f\) as the fitness score (\textit{lines 9-12}). If any \(f \geq \mathcal{L}_{\text{th}}\), the algorithm halts and returns that solution (\textit{lines 13-15}). Otherwise, iterations continue until the threshold or maximum generation \(g\) is reached.
Following fitness evaluation, solutions are ranked in descending order by fitness \(\mathbf{F}\) (\textit{line 17}). The top-ranking solution \(\mathbf{P}_{best}\) is preserved in the next generation \(\mathbf{P}_{new}\) to ensure elitism (\textit{line 19}). To populate the remaining slots in \(\mathbf{P}_{new}\), pairs of parent solutions are selected via tournament selection (\textit{line 21}). Crossover produces two offspring solutions from each parent pair (\textit{line 22}), and these offspring are then mutated at rate \(\mu\) to enhance solution diversity (\textit{line 23}). The mutated offspring are added to the new generation \(\mathbf{P}_{new}\) (\textit{line 24}). 
The updated population \( \mathbf{P}_{\text{new}} \) replaces \( \mathbf{P} \), and the cycle repeats until either \( g \) generations are completed or \( \mathcal{L}_{\text{th}} \) is met, at which point \( \mathbf{P}_{\text{best}} \) is returned as the optimal subset as the algorithm output.

% Algorithm \ref{algo:genetic} details the evolutionary optimization for weight-subset reduction. It begins by initializing parameters: subset size \( n \), population size \( m \), generation limit \( g \), and mutation rate \( \mu \) (\textit{line 1}). An initial population \( \mathcal{P} \) of \( m \) solutions is generated by selecting random subsets of \( n \) weights from the critical weight set \( \mathcal{W}_{\text{critical}} \) (\textit{line 2}). For each generation, the fitness of all solutions is evaluated relative to the target loss threshold \( L_{\text{th}} \) (\textit{line 4}), with solutions ranked in descending fitness order (\textit{line 5}). The top-ranked solution, \( S_{\text{best}} \), is preserved (elitism) for the next generation (\textit{line 6}). If \( L(S_{\text{best}}) \leq L_{\text{th}} \), the algorithm terminates, returning \( S_{\text{best}} \) (\textit{lines 7-8}). If not, a new generation \( \mathcal{P}_{\text{new}} \) is initialized with \( S_{\text{best}} \) (\textit{line 10}). Additional offsprings are generated by selecting two parent solutions through tournament selection (\textit{line 12}), applying a crossover to produce two offspring (\textit{line 13}), and mutating each offspring with probability \( \mu \) (\textit{line 14}). This process continues until \( \mathcal{P}_{\text{new}} \) reaches size \( m \) (\textit{lines 11-16}).
% The updated population \( \mathcal{P}_{\text{new}} \) replaces \( \mathcal{P} \), and the cycle repeats until either \( g \) generations are completed or \( L_{\text{th}} \) is met, at which point \( S_{\text{best}} \) is returned as the optimal subset (\textit{line 17}).

\subsubsection{Iterative Pruning-based Weight Set Reduction}\label{sec:adaptive_pruning}
After obtaining the optimized weight set from the genetic optimization process, we apply an iterative pruning-based reduction technique to further refine the weight set. This method systematically enhances the BFA efficiency by minimizing the weight set, iteratively removing elements with minimal impact on model performance. This approach leverages the insight that extensive solution spaces often contain redundant components, allowing non-critical elements to be pruned without diminishing attack effectiveness. By isolating only the most crucial weights, the iterative pruning optimization substantially reduces computational complexity, leading to a more streamlined and effective attack strategy.

\iffalse
\begin{algorithm}[t]
\caption{Iterative Pruning-based Weight Set Reduction}
\begin{algorithmic}[1]
\Require $\mathbf{W}$, Attack layer $l$, Best solution $\mathbf{P}_{best}$, Fitness score change limit $\epsilon$, maximum iterations $\mathcal{T}$, no-improvement threshold $\mathcal{N}$
\State Initialize no-improvement counter $c = 0$
\State $\mathbf{W}^{(l)} = \texttt{GetParams}(\mathbf{W},l)$
\State $I^{(l)}_{\text{hybrid}} \gets \mathbf{P}_{best}$
\State $\mathcal{L}_{best} \gets \texttt{BFLIP}
    ({\mathbf{W}^{(l)}, pos, I^{(l)}_{\text{hybrid}}})$
\For{$t = 1, 2, \dots, T$}
    \State $\mathbf{P}_{best_i} \gets \texttt{random.choice}(\mathbf{P}_{best})$
    \State $\mathbf{P}_{best}' \gets \mathbf{P}_{best} \setminus \{\mathbf{P}_{best_i}\}$\Comment{Remove index}
    \State $I^{(l)}_{\text{hybrid}} \gets \mathbf{P}_{best}'$
    \State $\mathcal{L} \gets \texttt{BFLIP}
    ({\mathbf{W}^{(l)}, pos, I^{(l)}_{\text{hybrid}}})$
    \If{$|\mathcal{L}_{best} - \mathcal{L}| < \epsilon$}
        \State $\mathbf{P}_{best} \gets \mathbf{P}_{best}'$
        \State $c \gets 0$ \Comment{Reset no-improvement counter}
    \Else
        \State $c \gets c+1$\Comment{Increment no-improvement counter}
    \EndIf
    \If{$c$ $\geq N$}
        \State \textbf{break}
    \EndIf
\EndFor
\State \Return $\mathbf{P}_{best}$
\end{algorithmic}
\label{algo:iterative}
\end{algorithm}
\fi

Our implementation is described as follows: Let the initial solution set be \( \mathbf{P}_{best} \) with initial loss \( \mathcal{L}_{best} \), defined as $\mathcal{L}_{best} = \mathcal{L}(\mathbf{P}_{best})$. For each iteration \( t \), up to a maximum \( T \), an index \( i \) is selected randomly from \( \mathbf{P}_{best} \) to form a temporary solution set \( \mathbf{P}_{best}' \) by removing \( \mathbf{P}_{best_i} \):
\begin{equation}
    \mathbf{P}_{best}' = \mathbf{P}_{best} \setminus \{ \mathbf{P}_{best_i} \}
\end{equation}
     
Following this, the loss \( \mathcal{L} \) is calculated  for \( \mathbf{P}_{best}' \):
\begin{equation}
    \mathcal{L} = \mathcal{L}(\mathbf{P}_{best}')
\end{equation}
If change in loss is greater than a threshold \( \epsilon \), update \( \mathbf{P}_{best} \)  with $\mathbf{P}_{best}'$ :
\begin{equation}
    \mathbf{P}_{best}  = \begin{cases} 
      \mathbf{P}_{best}' & \text{If } |\mathcal{L}_{best} - \mathcal{L}| < \epsilon  \\
      \mathbf{P}_{best} & \text{otherwise}.
   \end{cases}
\end{equation}
The process is terminated when \( T \) (pre-defined) iterations are reached or no improvement is observed over \( N \)(pre-defined) iterations.

Let us define the final solution as \( \mathbf{P}_{best}^* \). Then by construction for any solution index \( \mathbf{P}_{best_i} \in \mathbf{P}_{best}^* \):
\begin{equation}
    \mathcal{L}(\mathbf{P}_{best}^* \setminus \{ \mathbf{P}_{best_i} \}) - \mathcal{L}(\mathbf{P}_{best}^*) \geq \epsilon
\end{equation}

This implies that $\mathbf{P}_{best}^*$ is a locally optimal solution, representing the most simplified and efficient configuration under the given constraints.

% The iterative pruning-based weight set reduction technique is outlined in Algorithm \ref{algo:iterative}. It takes as input the model weights \( \mathbf{W} \), the attack layer \( l \), the best solution \( \mathbf{P}_{best} \), the fitness score change limit \( \epsilon \), the maximum number of iterations \( T \), and the no-improvement threshold \( N \). The algorithm begins by initializing a no-improvement counter \( c \) to zero (\textit{line 1}). It then collects the relevant model weights based on layer \( l \) (\textit{line 2}), along with the attack indices \( I^{(l)}_{\text{hybrid}} \) from \( \mathbf{P}_{best} \) (\textit{line 3}), and calculates the corresponding loss \( \mathcal{L}_{best} \) (\textit{line 4}).
% In each iteration, the algorithm selects a random index \( i \) from \( \mathbf{P}_{best} \) and removes it from the set (\textit{lines 6-7}). Using the updated set \( \mathbf{P}_{best}' \), the bit-flip perturbation loss \( \mathcal{L} \) is recalculated (\textit{lines 8-9}). If the difference between the new loss \( \mathcal{L} \) and the previous best loss \( \mathcal{L}_{best} \) is smaller than the threshold \( \epsilon \), the updated \( \mathbf{P}_{best}' \) is accepted as the new best solution, and the no-improvement counter \( c \) is reset (\textit{lines 10-12}). Otherwise, the no-improvement counter is incremented (\textit{line 15}). If the counter exceeds the threshold \( N \), the process terminates (\textit{lines 16-18}). If the maximum number of iterations \( T \) is not reached, the process continues until either the no-improvement threshold is surpassed or the iteration limit is exhausted. The algorithm outputs the reduced set \( \mathbf{P}_{best} \).

The iterative pruning-based weight set reduction technique, outlined in Algorithm \ref{algo:iterative}, takes as input model weights \( \mathbf{W} \), attack layer \( l \), best solution \( \mathbf{P}_{best} \), fitness score change limit \( \epsilon \), maximum iterations \( T \), and no-improvement threshold \( N \). The algorithm initializes the no-improvement counter \( c \) to 0 (\textit{line 1}), collects the relevant model weights for layer \( l \) (\textit{line 2}), attack indices from \( \mathbf{P}_{best} \) (\textit{line 3}), and calculates the initial loss \( \mathcal{L}_{best} \) (\textit{line 4}).

In each iteration, a random index \( i \) is selected from \( \mathbf{P}_{best} \) and removed (\textit{lines 6-7}). The bit-flip perturbation loss \( \mathcal{L} \) is recalculated for the updated solution (\textit{lines 8-9}). If the loss difference is less than \( \epsilon \), \( \mathbf{P}_{best}' \) is accepted, and the no-improvement counter is reset (\textit{lines 10-12}); otherwise, the counter is incremented (\textit{line 15}). If \( c \) exceeds \( N \), the process terminates (\textit{lines 16-18}), or it continues until the iteration limit \( T \) is reached. The final reduced \( \mathbf{P}_{best} \) is provided as the output.

This approach extracts the most optimal selection of weights from our genetically optimized solution, generating the most efficient attack vector for affecting the model performance through BFA.



==> sections/comparison.tex <==
\section{Efficiency against Existing Defenses}\label{sec:comparison}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t]
\centering
\caption{Effect of AttentionBreaker on existing defense.}
\label{tab:FaR_Table}
\renewcommand{\arraystretch}{1.5}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|cc|}
\hline
\rowcolor[HTML]{C0C0C0} 
\cellcolor[HTML]{C0C0C0} &
  \cellcolor[HTML]{C0C0C0} &
  \cellcolor[HTML]{C0C0C0} &
  \cellcolor[HTML]{C0C0C0} &
  \multicolumn{2}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Post-attack accuracy (\%)}} \\ \cline{5-6} 
\rowcolor[HTML]{C0C0C0} 
\multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{Model}} &
  \multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{Dataset}} &
  \multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Original \\ Accuracy (\%)\end{tabular}}} &
  \multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{\# of Bit-flips}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{With FaR}} &
  \textbf{Without FaR} \\ \hline \hline
 &
  CIFAR-100~\cite{krizhevsky2009learning} &
  91.55 &
  224 &
  \multicolumn{1}{c|}{3.4} &
  4.2 \\ \cline{2-6} 
\multirow{-2}{*}{ViT} &
  ImageNet1k~\cite{russakovsky2015imagenet} &
  80.1 &
  268 &
  \multicolumn{1}{c|}{10.9} &
  10.2 \\ \hline
\end{tabular}%
}
\end{table}

% \subsection{Against Forget and Rewire (FaR)}
% \textbf{Forget and Rewire (FaR) Framework: Limitations and Vulnerabilities in Enhancing Transformer Resilience Against Bit-Flip Attacks}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
Forget and Rewire (FaR), inspired by ``brain rewiring,'' is a defense against bit-flip attacks, previously explored in small-scale vision tasks but not in generative tasks with LLMs. FaR enhances Transformer robustness by redistributing tasks from critical to less essential neurons in linear layers, reducing sensitivity to bit flips and hindering gradient-based adversarial methods~\cite{nazari2024forget}. However, this approach fails against gradient-free techniques like AttentionBreaker, which remain effective even without gradient reliance (see Section \ref{sec:gradfree}).


% there exist one potential defense that were explored in the context of only vision small scale tasks, unlike us where we explore on generative task using LLM
% Existing research in this direction comprises the Forget and Rewire (FaR) framework, inspired by `brain rewiring,' which aims to bolster Transformer robustness against bit-flip attacks by adjusting neuron connectivity within linear layers~\cite{nazari2024forget}. This framework leverages the unique architecture of Transformers, concentrating on the selective redistribution of connections within these layers. FaR specifically reallocates tasks from critical to less essential neurons, reducing the model’s reliance on particular parameters and theoretically decreasing sensitivity to bit flips while obfuscating essential parameters from gradient-based adversarial algorithms. FaR aims to shield key parameters by focusing on linear layers, enhancing resilience against random bit-flip attacks. \emph{However, this sensitivity redistribution approach by FaR does not protect against the gradient-free AttentionBreaker technique, which remains effective without relying on gradients (see Section \ref{sec:gradfree}).}

To illustrate FaR's limitations, we applied AttentionBreaker to a ViT-Base~\cite{dosovitskiy2020vit} model utilized in FaR demonstrations. Our results reveal that, despite the FaR defense, the model remains highly susceptible, with accuracy on the ImageNet1k dataset plummeting from 80.7\% to 10.9\% after just 268 (\(\approx 3 \times 10^-6\)\%) bit-flips as captured in Table \ref{tab:FaR_Table}. This highlights the FaR framework's shortcomings in providing robust protection across model layers.
%However, restricting defense mechanisms to linear layers is inherently limiting, as other layers—such as attention layers—are also highly susceptible to adversarial bit-flips, as demonstrated in our analysis. This narrow focus not only leaves vulnerabilities across other model layers unaddressed but may also lead users to assume comprehensive protection, potentially resulting in complacency and critical oversights in model security.
